Enhance Low-Carbon Power System Operation via Carbon-Aware Demand Response

As the electrification process advances, enormous power flexibility is becoming available on the demand side, which can be harnessed to facilitate power system decarbonization. Hence, this paper studies the carbon-aware demand response (C-DR) paradigm, where individual users aim to minimize their carbon footprints through the optimal scheduling of flexible load devices. The specific operational dynamics and constraints of deferrable loads and thermostatically controlled loads are considered, and the carbon emission flow method is employed to determine users' carbon footprints using nodal carbon intensities. Then, an optimal power dispatch model that integrates the C-DR mechanism is proposed for low-carbon power system operation, based on the carbon-aware optimal power flow (C-OPF) method. Two solution algorithms, including a centralized Karush-Kuhn-Tucker (KKT) reformulation algorithm and an iterative solution algorithm, are developed to solve the bi-level power dispatch optimization model. Numerical simulations on the IEEE New England 39-bus system demonstrate the effectiveness of the proposed methods.

==> Biogra.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{XinChen.jpg}}]{Xin Chen} is an Assistant Professor in the Department of Electrical and Computer Engineering at Texas A\&M University. Prior to joining TAMU, he was a Postdoctoral Associate affiliated with MIT Energy Initiative at Massachusetts Institute of Technology. He received the Ph.D. degree in electrical engineering from Harvard University, the master’s degree in electrical engineering and two bachelor’s degrees in engineering and economics from Tsinghua University. Dr. Chen is a recipient of the IEEE PES Outstanding Doctoral Dissertation, IEEE Transactions on Smart Grid Top-5 Papers, the Best Research Award at the 2023 IEEE PES Grid Edge Conference, the Outstanding Student Paper Award at the 2021 IEEE Conference on Decision and Control,  the Best Student Paper Award Finalist at the 2018 IEEE Conference on Control Technology and Applications, and the Best Conference Paper Award at the 2016 IEEE PES General Meeting.
\end{IEEEbiography}

 
